Better Embeddings with Coupled Adam

Despite their remarkable capabilities, LLMs learn word representations that exhibit the undesirable yet poorly understood feature of anisotropy. In this paper, we argue that the second moment in Adam is a cause of anisotropic embeddings, and suggest a modified optimizer called Coupled Adam to mitigate the problem. Our experiments demonstrate that Coupled Adam significantly improves the quality of embeddings, while also leading to better upstream and downstream performance on large enough datasets.

==> header/definitions.tex <==
\newcommand{\M}{\rm M}
\newcommand{\B}{\rm B}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}

\newcommand{\tm}{\tau}  %
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{{\rm I}} %
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\Acc}{\rm Acc}
\newcommand{\ISO}{{\rm Iso}}
\newcommand{\munorm}{\|\mu\|}
\newcommand{\munormrel}{\|\mu\|^{\rm r}}
\newcommand{\rcos}{\overline{r}}
\newcommand{\V}{\mathcal{V}}
\def\colhighlight{ForestGreen}
\newcommand{\highlight}[1]{{\color{\colhighlight} #1}}
\newcommand{\firstmoment}{\widehat{m}_i^{(\tm)}}
\newcommand{\secondmoment}{\widehat{v}_i^{(\tm)}}
\newcommand{\secondmomentavg}{\widehat{\nu}^{(\tm)}}
\newcommand{\secondmomentshort}{\widehat{v}_i}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

